Frequency Automata: A novel formal model of hybrid systems in combined time and frequency domains

Hybrid systems are mostly modelled, simulated, and verified in the time domain by computer scientists. Engineers, however, use both frequency and time domain modelling due to their distinct advantages. For example, frequency domain modelling is better suited for control systems, using features such as spectra of the signal. Considering this, we introduce, for the first time, a formal model called frequency automata for hybrid systems modelling and simulation, which are represented in combined time and frequency domains. We propose a sound translation from Hybrid Automata (HA) to Frequency Automata (FA). We also develop a numerical simulator for FA and compare it with the performance of HA. Our approach provides precise level crossing detection and efficient simulation of hybrid systems. We provide empirical results comparing simulation of HA via its translation to FA and its simulation via Matlab Simulink/Stateflow. The results show clear superiority of the proposed technique with the execution times of the proposed technique 118x to 1129x faster compared to Simulink/Stateflow. Moreover, we also observe that the proposed technique is able to detect level crossing with complex guards (including equality), which Simulink/Stateflow fail.

==> figures/cartesian.tex <==
\begin{tikzpicture}
  % First plot: Rotating vector
  \begin{scope}[shift={(-3,0)}] % Move to the left to fit the second graph
    % Draw x-axis and y-axis
    \draw[->] (-2,0) -- (2,0) node[right] {$x$};
    \draw[->] (0,-2) -- (0,2) node[above] {$y$};
    
    % Draw initial vector (gray, reference along x-axis)
    \draw[thick, ->, gray] (0,0) -- (1.5,0);
    
    % Draw rotated vector (example: π/4)
    \draw[thick, ->, blue] (0,0) -- ({1.5*cos(45)}, {1.5*sin(45)}) node[above right] {$\vec{v}$};
    
    % Draw angle arc with an arrow to indicate rotation
    \draw[thick, red, ->] (1,0) arc[start angle=0, end angle=45, radius=1];
    
    % Label the angle in terms of π
    \node at ({1.2*cos(22.5)}, {1.2*sin(22.5)}) [red] {$d\theta$};
  \end{scope}
  
  % Second plot: Arbitrary signal
  \begin{axis}[
    at={(5cm,0)}, % Shift to the right
    width=6cm, height=4cm,
    axis x line=middle,
    axis y line=middle,
    xlabel={$t$},
    ylabel={Signal},
    samples=100,
    domain=0:2
    ]
    % Arbitrary signal between 0 and sin(pi/4)
    \addplot[thick, purple] {sin(deg(x)) * sin(deg(45))};
  \end{axis}
  
\end{tikzpicture}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> figures/stwheelproof.tex <==
\begin{tikzpicture}[
	% as the function is used more than once, make a shorthand
	declare function={
	%	f(\x)=10000/(9999*e^(-0.125*\x)+10)+100;
	f(\x)=1*sin(deg(\x));
	f2(\x)=\x;
	}
	]
	\begin{axis}[
		name=ax1,
		axis lines=middle,
		xlabel=$\theta$,
		ylabel=$x$,
		grid=major,
		samples=100,
		domain=-pi/2:pi/2,
		xtick={-pi/2, 0, pi/2, pi, 3*pi/2},
		xticklabels={$-\frac{\pi}{2}$, $0$, $\frac{\pi}{2}$, $\pi$, $\frac{3\pi}{2}$}
		]
		
			% Plot the cosine function
		\addplot[blue, thick] {sin(deg(x))};
		\addplot[domain=-0.4:0.4, red, thick, smooth] {f2(x)};
			
		% define coordinates at bottom left and top left of rectangle
		\coordinate (c1) at (axis cs:0.0,0.0);
		\coordinate (c2) at (axis cs:0.0,0.1);
		% draw a rectangle
		\draw (c1) rectangle (axis cs:0.1,0.1);
		
		
	\end{axis}
	
	\begin{axis}[
		name=ax2,
		scaled ticks=false,
		yticklabel=\empty,
		xticklabel=\empty,
		%xmin=0,xmax=2,
		%ymin=0,ymax=2,
		xlabel=$\theta$,
		ylabel=$\sin(\theta)$,
		% place second axis relative to first one
		% anchor is south west
		at={($(ax1.south east)+(2cm,0)$)},
		% turn on grid
		xmajorgrids=true,
		grid style={help lines,dashed},
		% to avoid clipping of a...e nodes
		clip=false,
		%domain = 0:0.3,
		]

		\addplot[domain=0:0.3, blue, ultra thick,smooth] {f(x)};
	

		
	\end{axis}
	

	
	% draw dashed lines from rectangle in first axis to corners of second
	\draw [dashed] (c1) -- (ax2.south west);
	\draw [dashed] (c2) -- (ax2.north west);
\end{tikzpicture}

==> figures/stwheelsimul.tex <==
    \begin{tikzpicture}
	\begin{axis}[
		axis lines=middle,
		xlabel=$x$,
		ylabel=$\cos(x)$,
		grid=major,
		samples=100,
		domain=-pi/2:3*pi/2,
		xtick={-pi/2, 0, pi/2, pi, 3*pi/2},
		xticklabels={$-\frac{\pi}{2}$, $0$, $\frac{\pi}{2}$, $\pi$, $\frac{3\pi}{2}$}
		]
		% Plot the cosine function
		\addplot[blue, thick] {cos(deg(x))};
		
		% Faster vertical sine wave starting at x = pi/2
		\addplot[green, thick, domain=-1:1, samples=200] ({pi/2 + 1.2*sin(4 * deg(x))}, x);
		
		% Draw a vertical line from leftmost peak of sine to cosine
		\draw[dashed, red] 
		(axis cs:{pi/2 + 1.2}, {0.4}) -- 
		(axis cs:{pi/2 + 1.2}, {-0.9 });
		
		\draw[dashed, red] 
		(axis cs:{ 0.35}, {0.9}) -- 
		(axis cs:{ 0.35}, {-0.4 });
		
		\node[right, red] at (axis cs:{pi/2 + 1.2}, {0.4}) {$\arcsin(-0.99)$};
		\node[right, red] at (axis cs:{0.35}, {0.4}) {$\arcsin(0.99)$};
		
		% Label it as "Initial"
	            \addplot[red, only marks, mark=*] coordinates {(pi/2, 0)};
	\node[red, anchor=north] at (axis cs:pi/2, 0.2) {Initial};
		
	\end{axis}
\end{tikzpicture}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

